Tracing the Propagation Path: A Flow Perspective of Representation Learning on Graphs

Graph Convolutional Networks (GCNs) have gained significant developments in representation learning on graphs. However, current GCNs suffer from two common challenges: 1) GCNs are only effective with shallow structures; stacking multiple GCN layers will lead to over-smoothing. 2) GCNs do not scale well with large, dense graphs due to the recursive neighborhood expansion. We generalize the propagation strategies of current GCNs as a \emph{"Sink$\to$Source"} mode, which seems to be an underlying cause of the two challenges. To address these issues intrinsically, in this paper, we study the information propagation mechanism in a \emph{"Source$\to$Sink"} mode. We introduce a new concept "information flow path" that explicitly defines where information originates and how it diffuses. Then a novel framework, namely Flow Graph Network (FlowGN), is proposed to learn node representations. FlowGN is computationally efficient and flexible in propagation strategies. Moreover, FlowGN decouples the layer structure from the information propagation process, removing the interior constraint of applying deep structures in traditional GCNs. Further experiments on public datasets demonstrate the superiority of FlowGN against state-of-the-art GCNs.

==> appedix.tex <==
% !TEX root = 19-0.tex
\section{Appendix}
\subsection{Proof of Theorem 4.1}\label{proof4.1}
To prove Theorem 4.1, we describe some preliminaries. Our proof partially relies on the results given by \cite{xu2018representation}, where the authors . For completeness, we give the definition of influence distribution and the theorem.

 
\begin{definition}[Influence score and distribution]
Given a graph  $\mathcal{G(V,E)}$, let $h_{x}^{(0)}$ be the input feature and $h_{x}^{(k)}$ be the learned hidden feature of node $x \in \mathcal{V}$ at the k-th layer of the model. The \emph{influence score} $I(x,y)$ of node $x$ by any node  $y \in \mathcal{V}$ is the sum of the absolute values of the entries of the Jacobian matrix $[\frac{\partial h_{x}^{(k)}}{\partial h_{y}^{(0)}}]$. We define the \emph{influence distribution} $I_{x}$ of $x \in \mathcal{V}$ by normalizing the \emph{influence scores}: $I_{x}(y)=I(x,y)/ \sum_{z}I(x,z)$, or $I_{x}(y)= e^{T}[\frac{\partial h_{x}^{(k)}}{\partial h_{y}^{(0)}}] e / (\sum_{z\in V}e^{T} [\frac{\partial h_{x}^{(k)}}{\partial h_{z}^{(0)}}] e )$, where $e$ is the all-ones vector. 
\end{definition}
\begin{theorem}\label{app:theoremjk}
Given a k-layer GCN with averaging as its neighborhood aggregation scheme, assume that all paths in the computation graph of the model are activated with the same probability of success $\rho$. Then the influence distribution $I_{x}$ for any node $x \in \mathcal{V}$ is equivalent, in expectation, to the $k$-step random walk distribution on the same graph stating at node $x$.
\end{theorem}


Below we restate the Theorem 4.1 and provide a proof.
\renewcommand{\thetheorem}{\ref{t1}}
\begin{theorem}\label{app:t1}
Given a grid graph $\mathcal{G(V,E)}$, and a k-layer GCN with averaging as its neighborhood aggregation scheme, there exists an equivalent version of \method{} that has the same influence distribution for every node $x \in \mathcal{V}$. 
\end{theorem}

\begin{proof}
We prove Theorem 4.1 in three steps. First, we prove that the influence distribution of a k-layer GCNs with averaging as its neighborhood aggregation scheme is equivalent to a k-step random walker with uniform transition probabilities. This can directly inferred from Theorem \ref{app:theoremjk} and its proof \citep{xu2018representation}. 

Second, a random walker with uniform transition probabilities in a grid graph indicates that every node has a same number of neighbors and a same transition probability to its neighbors. In other words, the random walker is symmetric and so is the related influence distribution of GCNs, i.e, $I_{x}(y) = I_{y}(x)$. 

Third, we prove that there exists a one-layer FlowGN that its influence distribution is equivalent to a k-step random walker. We can set the return parameter $p=1$, the in-out parameter $q=1$, and the path length $l=k$ so the generated flow paths are exactly a sampling of a k-step random walker (in grid graphs the importance of all nodes are the same in a structural view). We apply the same information propagation mechanism used in the experiments, i.e., $GenerateFlow(s)=h_{s}$, $TransmitFlow(v_{i}, flow)=flow$, and $ConserveFlow(v_{i},flow)= flow$. For clarification, we set \emph{source} node as $y$ and \emph{sink} node as $y$. Following the proof procedure of Theorem \ref{app:theoremjk} \citep{xu2018representation}, we can draw that $E[\frac{\partial h_{y}^{(k)}}{\partial h_{x}^{(0)}}] = \rho \cdot W \cdot (\prod^{\Phi}_{p=1} \prod_{l=k}^{1}\frac{1}{\widetilde{deg}(v_{p}^{l})})$. By normalizing the distribution scores, we can get that the influence distribution $I_{x}(y)$ of FlowGN is equivalent to a random walker that starts at node $y$. Since $I_{x}(y) = I_{y}(x)$, we get the Theorem proved.


\end{proof}

 \subsection{Experimental Details} \label{app:exp}
 
 We used TensorFlow for all experiments except SGC, which is implemented by Pytorch.  Running time is compared on a single machine with 4-core 2.2 GHz Intel Core i7, and 16G RAM. For FlowGN, we set weight decay to $0.00001$, epochs to $30$ hidden and out dimensions to $50$ The early stopping criterion uses a patience of $p = 10$ and epochs is set to $100$. The learning rate is set to $0.0001$. 
 
We mainly use the original parameters for baselines. The vanilla GCN uses the original settings of two layers with $h = 16$ hidden units, no dropout on the adjacency matrix, $L_2$ regularization parameter $\lambda = \num{5e-4}$ and the original early stopping with a maximum of 200 steps and a patience of 10 steps based on the loss. The batch version of GCN is the same as the one used by FastGCN. For GAT and SGC, we use the (well optimized) original hyperparameters. For GraphSAGE, we set batch size to $256$ and dropout to $0$. In Section 5.3, due to memory limit, we set the sampling size to $5$ and batch size to $50$ for all layers when model depth exceeds $5$. For FastGCN, the sampling size is set to $400$.

\subsection{Additional Experimental Results}

Results of Cora are shown in Figure \ref{app:r-l path} and Figure \ref{app:cora2}. The optimal $l$ is $6$ and optimal $q$ is $0.1$, and we can get similar conclusion as what we made in Section 5.2.
\begin{figure}[th ]
\centering
\begin{subfigure}{.3\textwidth}
\includegraphics[height=4cm]{flowpath_cora.pdf}
 \caption{Cora}
\end{subfigure}
%\includegraphics{SERecmodel1.pdf}
\caption{Prediction accuracy of FlowGN with different path length $l$ and in-out parameter $q$.}
\label{app:r-l path}
\end{figure}

\begin{figure}
%--1st pic--
\centering 
\begin{tikzpicture}[scale=0.6]
\begin{axis}[
    xlabel={$\mathcal{K}$ },
    %ylabel={F1 score},
    xmin=1, xmax=7,
    ymin=0.43, ymax=0.9,
    xtick={1,2,3,4,5,6,7},
    ytick={0,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1 },
    legend pos=south west,
    ymajorgrids=true,
    grid style=dashed,
]
  \addplot[
    color=red,
    mark=*,
    line width=1pt,
    ]
    coordinates {
    (1,0.78400)(2,0.83205)(3,0.84778)(4,0.84546)(5,0.86312)(6,0.84590)(7,0.84624) 
    %(1, 0.842)(2, 0.87)(3, 0.869)(4, 0.865)(5, 0.859)(6, 0.851)(7, 0.845)
    };
    \addlegendentry{FlowGN}
    
        \addplot[
    color=violet,
    mark=diamond,
    line width=2pt,
    ]
    coordinates {
   (1,0.5207)(2,0.8220)(3,0.76817)(4, 0.7410)(5,0.7269)(6, 0.7079)(7,0.6732)
    };
   \addlegendentry{GraphSAGE}   
   
\addplot[
    color=cyan,
    mark=asterisk,
    line width=2pt,
    ]
    coordinates {
(1,0.58700)(2,0.86300)(3,0.86000)(4,0.84600)(5,0.79300)(6,0.51600)(7,0.44300)
    };
   \addlegendentry{GCN}
 \addplot[
    color=blue,
    mark=square,
    line width=1pt,
    ]
    coordinates {
    (1, 0.842)(2, 0.87)(3, 0.869)(4, 0.865)(5, 0.859)(6, 0.851)(7, 0.845)
    };
    \addlegendentry{SGC}
    
\end{axis}
\end{tikzpicture}
\caption{Prediction accuracy of FlowGN on \emph{Cora} with different layer numbers $\mathcal{K}$}\label{app:cora2}
\end{figure}
 
 


\iffalse
\subsection{Discussion}
\textbf{Relation between importance sampling, centrality measure and network flow.}
The FastGCN shows that importance sampling consistently yields higher accuracy than does uniform sampling.
 
\textbf{Feature Propagation and Network Flow.}  
The standard aggregation method implicitly assumes the features flow among nodes with equal probability. Multiplication of adjacency matrix of the graph.

assume neighboring nodes have similar representations, which may cause the over-smoothing problem

\textbf{Scalability and extensibility.} FlowGN compared
easy to applied to parallel computing,
\fi 
